Integrating Subgraph-aware Relation and DirectionReasoning for Question Answering

Question Answering (QA) models over Knowledge Bases (KBs) are capable of providing more precise answers by utilizing relation information among entities. Although effective, most of these models solely rely on fixed relation representations to obtain answers for different question-related KB subgraphs. Hence, the rich structured information of these subgraphs may be overlooked by the relation representation vectors. Meanwhile, the direction information of reasoning, which has been proven effective for the answer prediction on graphs, has not been fully explored in existing work. To address these challenges, we propose a novel neural model, Relation-updated Direction-guided Answer Selector (RDAS), which converts relations in each subgraph to additional nodes to learn structure information. Additionally, we utilize direction information to enhance the reasoning ability. Experimental results show that our model yields substantial improvements on two widely used datasets.

==> related.tex <==
\section{Related Work}

\noindent \textbf{Question Answering Models}

\noindent KB-based question answering models are mainly divided into two forms: semantic parsing and deep learning models.  Among the semantic parsing-related studies, \citet{DBLP:conf/acl/YihHM14} focus on single-relation questions and decomposes each question into an entity mention and a relation pattern. \citet{DBLP:conf/acl/YihRMCS16} show the value of collecting semantic parse labels for knowledge base question answering. Among the deep learning approaches, \citet{DBLP:conf/emnlp/YavuzGSY17} propose a continuous checking mechanism to judge the correctness of answer evidence. \citet{DBLP:conf/aaai/ZhangDKSS18} propose variational learning algorithm to perform multi-hop reasoning. \citet{DBLP:conf/aaai/WangKMYTACFMMW19} explore additional knowledge bases to improve natural language inference. \citet{DBLP:conf/aaai/MitraCTB19} translate the question and the natural language text to a logical representation and then use logical reasoning. Compared with the semantic parsing, deep learning models need less additional feature engineering and can be trained in an end-to-end fashion. 
Previous models mainly focus on single-answer prediction \cite{survey} and choose the correct answer from the candidates based on the ranking method. However, the usage of the ranking method in a multi-answer prediction scenario isn't straightforward, because the multi-answer prediction performance is affected by the threshold value, which is hard to estimate \cite{DBLP:conf/emnlp/SunDZMSC18}.



In a question-specific subgraph, to utilize the relation information and help with the reasoning, \citet{DBLP:conf/emnlp/SunDZMSC18} update entity representations by considering weighted summation of neighbor entity information based on the similarity of edges (relations) and the question. 
\citet{DBLP:conf/coling/SorokinG18} consider utilizing relation information of the subgraph to encode the structure of the question. These models' understanding of the relation information remains poor, since they adopt the fixed relation representations across different subgraphs, resulting in a failure to fully capture subgraph structured information. 

\noindent \textbf{Levi Graph}

\noindent \citet{gross2004handbook} propose Levi Graph which transforms edges to additional nodes to make them learnable and capture rich structured information. \citet{ribeiro2019enhancing,DBLP:conf/acl/CohnHB18} employ Levi Graph to the task of generating text from graph-based data, demonstrating that Levi Graph has a strong ability to encode relation representations.

\noindent \textbf{Graph Convolution Networks}

\noindent  Supported with a number of studies on graph representation learning \cite{Kipf2016Semi,DBLP:conf/esws/SchlichtkrullKB18,DBLP:conf/www/WangJSWYCY19}, graph convolution network (GCN) shows its powerful ability in graph analysis. A massive number of GCN-based algorithms are designed to perform reasoning over graphs, such as R-GCN \cite{DBLP:conf/esws/SchlichtkrullKB18}, GRAFT-Net \cite{DBLP:conf/emnlp/SunDZMSC18}, and BAG \cite{DBLP:conf/naacl/CaoFT19}. The GCN enables information flow along the direction of the edge between two adjacent nodes to update the node representations, which simulates the reasoning process. However, as shown in Figure~\ref{example}(b), the direction of this information propagation may be inconsistent with the direction of human reasoning \cite{johnson2012inference}, which can affect the reasoning performance.





 


